Three-dimensional Simulations and Synthetic Polarization of the SS 433 Jet

Context. SS 433 is the prototypical microquasar and the only known Galactic system hosting persistent, precessing relativistic jets powered by supercritical accretion. Recent X-ray polarimetric observations have revealed highly ordered magnetic fields and station- ary high-energy emission regions that are likely associated with recollimation shocks. Aims. We investigate how magnetic-field topology influences the formation of recollimation shocks, jet morphology, and polarized synchrotron emission in SS 433-like jets, with the goal of constraining the magnetic structure responsible for the observed X-ray polarization. Methods. We performed a suite of three-dimensional relativistic magnetohydrodynamic simulations using the PLUTO code, exploring purely poloidal, purely toroidal, and mixed helical magnetic-field configurations. The resulting magnetic and thermodynamic struc- tures were post-processed with the polarized radiative-transfer code 3DPol to generate synthetic synchrotron intensity and polarization maps directly comparable to observations. Results. We find that the magnetic topology is the primary regulator of jet collimation and shock development. Toroidal-field jets produce the narrowest outflows and the strongest sequence of recollimation shocks, whereas poloidal-field jets remain broader and dynamically smoother. The large-scale polarization structure is remarkably insensitive to jet radius and non-thermal particle normal- ization. Instead, the polarization signatures are governed almost entirely by the magnetic geometry. Poloidal-dominated configurations produce high and stable polarization fractions, supported by the IXPE observations of SS 433, with magnetic fields aligned with the jet direction, whereas toroidal-dominated models generate more complex polarization structures and transverse signatures.

==> fig1_ss433_sketch.tex <==
%% Fig. 1 — Schematic of the SS 433 / W50 system
%% Requires: \usepackage{tikz} in the preamble
%% Optional but recommended: \usetikzlibrary{arrows.meta}
%%
%% Coordinate system: 1 TikZ unit = 10 pc; SS 433 binary at origin.
%% East = +x; North = +y.  Jet half-opening angle 10 deg,
%% so half-width at distance d (units) = d*tan(10 deg) ~ 0.176*d.
%%
%% Adjust the overall [scale=...] to fit your column width.
%% At scale=0.68 the figure is ~18 cm wide (two-column A&A).

\begin{figure*}
\centering
\begin{tikzpicture}[
  scale  = 0.68,
  >=latex,                          % arrowhead style
  every node/.style = {font=\small} % base font
]

% ------------------------------------------------------------------
% W50 NEBULA BOUNDARY  (ear-shaped dashed contour)
% ------------------------------------------------------------------
% Eastern ear: base ~3.5 units N/S of axis, tip rounded at x~10
\draw[gray!75, dashed, semithick]
  (0, 3.5)
    .. controls (3.5, 5.2) and (7.0, 4.2) .. (9.8,  0.6)
    .. controls (10.4, 0.2) and (10.4,-0.2) .. (9.8, -0.6)
    .. controls (7.0,-4.2) and (3.5,-5.2) ..
  (0,-3.5);
% Western ear (mirror image)
\draw[gray!75, dashed, semithick]
  (0, 3.5)
    .. controls (-3.5, 5.2) and (-7.0, 4.2) .. (-9.8,  0.6)
    .. controls (-10.4, 0.2) and (-10.4,-0.2) .. (-9.8,-0.6)
    .. controls (-7.0,-4.2) and (-3.5,-5.2) ..
  (0,-3.5);
% Labels
\node[gray!75, font=\itshape\footnotesize] at ( 11.0, 0) {W50};
\node[gray!75, font=\itshape\footnotesize] at (-11.0, 0) {W50};

% ------------------------------------------------------------------
% LARGE-SCALE COLLIMATED JET
% Half-width at d units from binary: 0.1763*d  (tan 10 deg)
% Eastern jet: inner edge at 10 pc (x=1), outer at 120 pc (x=12)
%   upper/lower edges: (1, +/-0.176) -- (12, +/-2.116)
% ------------------------------------------------------------------
% Filled jet bodies
\fill[blue!10]
  (1, 0.176) -- (12, 2.116) -- (12,-2.116) -- (1,-0.176) -- cycle;
\fill[blue!10]
  (-1, 0.176) -- (-12, 2.116) -- (-12,-2.116) -- (-1,-0.176) -- cycle;
% Jet boundary lines
\draw[blue!55!black, semithick] (1, 0.176) -- (12, 2.116);
\draw[blue!55!black, semithick] (1,-0.176) -- (12,-2.116);
\draw[blue!55!black, semithick] (-1, 0.176) -- (-12, 2.116);
\draw[blue!55!black, semithick] (-1,-0.176) -- (-12,-2.116);
% Jet axes (dashed with arrow on eastern side)
\draw[blue!55!black, dashed, thin, ->] (0, 0) -- (13.2, 0);
\draw[blue!55!black, dashed, thin    ] (0, 0) -- (-12.8, 0);
% Jet label
\node[blue!55!black, font=\footnotesize, anchor=south west] at (8.2, 2.5)
  {relativistic jet};
\node[gray!70, font=\scriptsize, anchor=north west] at (8.2, 2.5)
  {($\beta = 0.26\,c$)};

% ------------------------------------------------------------------
% HALF-OPENING ANGLE ANNOTATION
% Arc at origin from 0 to 10 deg, radius 2.0; tick at x=5
% ------------------------------------------------------------------
\draw[gray!65, thin] (2.0, 0) arc (0:10:2.0);   % arc from (2,0) centred at origin
\draw[gray!55, dashed, very thin] (5, 0) -- (5, 0.882); % tick to upper edge at 50 pc
\node[gray!65, font=\scriptsize, anchor=west] at (2.15, 0.32)
  {$\theta \approx 10^{\circ}$};

% ------------------------------------------------------------------
% INNER PRECESSING JET CONE  (schematic; true extent << 1 pc)
% Shown as a narrow wedge, half-angle ~20 deg, length ~1 unit
% ------------------------------------------------------------------
\fill[violet!18!white] (0,0) -- ( 1.0, 0.40) -- ( 1.0,-0.40) -- cycle;
\draw[violet!60!black, thin] (0,0) -- ( 1.0, 0.40)
                              (0,0) -- ( 1.0,-0.40);
\fill[violet!18!white] (0,0) -- (-1.0, 0.40) -- (-1.0,-0.40) -- cycle;
\draw[violet!60!black, thin] (0,0) -- (-1.0, 0.40)
                              (0,0) -- (-1.0,-0.40);
% Leader + label (upper right of the eastern cone tip)
\draw[gray!60, thin] (1.0, 0.40) -- (1.5, 0.80);
\node[violet!65!black, font=\scriptsize, anchor=south west] at (1.55, 0.80)
  {precessing inner jet (schematic; $<\!1\,$pc)};

% ------------------------------------------------------------------
% CENTRAL BINARY SYSTEM
% ------------------------------------------------------------------
% Accretion disc (edge-on ellipse)
\draw[gray!55, thin] (0,0) ellipse (0.65 and 0.13);
% Donor star (A-type supergiant): filled orange circle
\fill[orange!75!yellow] (-0.23, 0) circle (0.30);
\draw[black, thin      ] (-0.23, 0) circle (0.30);
% Compact object (BH/NS): open circle with cross
\fill[white            ] ( 0.28, 0) circle (0.22);
\draw[black, semithick ] ( 0.28, 0) circle (0.22);
\draw[black, thin      ] ( 0.07, 0) -- (0.49, 0);
\draw[black, thin      ] ( 0.28,-0.22) -- (0.28, 0.22);
% Labels
\node[font=\small\bfseries, anchor=south] at (0, 0.44) {SS\,433};
\node[gray!65, font=\scriptsize, anchor=north] at (0,-0.50)
  {(A-type star + BH/NS)};

% ------------------------------------------------------------------
% RECOLLIMATION SHOCK KNOTS  at 30 pc (x=3)
% Jet half-width at x=3: 0.529 units
% ------------------------------------------------------------------
% Shock front bar (vertical, slightly wider than jet)
\draw[red!55!black, very thick] (3,-0.72) -- (3, 0.72);

% IXPE marker: filled red diamond (lozenge)
\fill[red!60!black]
  (3.0, 0.52) -- (3.18, 0.34) -- (3.0, 0.16) -- (2.82, 0.34) -- cycle;

% NuSTAR marker: filled blue circle
\fill[blue!65!black] (3.0,-0.06) circle (0.17);

% HAWC marker: open green triangle (pointing up)
\draw[green!55!black, semithick]
  (2.83,-0.50) -- (3.00,-0.22) -- (3.17,-0.50) -- cycle;

% Leader line and labels
\draw[gray!60, thin] (3, 0.75) -- (3, 1.45);
\node[font=\small\bfseries, anchor=south] at (3, 1.45) {e1\,/\,C11};
\draw[gray!60, thin] (3, 3.90) -- (3, 2.65);
\node[gray!65, font=\scriptsize, anchor=south] at (3, 2.65)
  {\textit{(recollimation shock)}};

% Distance annotation: binary to knot
\draw[<->, gray!65, thin] (0.05,-1.05) -- (2.95,-1.05);
\node[gray!65, font=\scriptsize] at (1.5,-1.30) {$\sim\!30\,$pc};

% ------------------------------------------------------------------
% SIMULATION DOMAIN ARROW  (10-120 pc, eastern side)
% ------------------------------------------------------------------
\draw[<->, semithick] (1,-4.8) -- (12,-4.8);
\draw[thin] ( 1,-4.4) -- ( 1,-5.2);
\draw[thin] (12,-4.4) -- (12,-5.2);
% Drop-lines from inner/outer domain limits to arrow
\draw[gray!55, dashed, very thin] ( 1,-2.6) -- ( 1,-4.7);
\draw[gray!55, dashed, very thin] (12,-3.0) -- (12,-4.7);
% Labels
\node[font=\small\bfseries, anchor=north] at (6.5,-4.8)
  {simulation domain};
\node[gray!65, font=\scriptsize, anchor=north] at (6.5,-5.3)
  {($\sim\!10$--$120\,$pc from SS\,433)};

% ------------------------------------------------------------------
% SCALE BAR  (10 pc = 1 unit), lower right
% ------------------------------------------------------------------
\draw[very thick] (10.0,-6.3) -- (11.0,-6.3);
\draw[semithick]  (10.0,-6.0) -- (10.0,-6.6);
\draw[semithick]  (11.0,-6.0) -- (11.0,-6.6);
\node[font=\footnotesize, anchor=north] at (10.5,-6.6) {10\,pc};

% ------------------------------------------------------------------
% NORTH ARROW, lower right
% ------------------------------------------------------------------
\draw[->, very thick] (12.5,-6.6) -- (12.5,-5.6);
\node[font=\footnotesize, anchor=north] at (12.5,-6.7) {N};

% ------------------------------------------------------------------
% EAST / WEST DIRECTION LABELS
% ------------------------------------------------------------------
\node[gray!65, font=\footnotesize\bfseries] at ( 13.5, 0) {E};
\node[gray!65, font=\footnotesize\bfseries] at (-13.5, 0) {W};

% ------------------------------------------------------------------
% LEGEND  (lower left, inside western W50 ear area)
% ------------------------------------------------------------------
\begin{scope}[shift={(-12.8,-1.8)}]
  % Box
  \draw[gray!60, thin, rounded corners=3pt]
    (-0.2, 0.8) rectangle (4.5,-2.8);
  % IXPE
  \fill[red!60!black]
    (0.20, 0.52) -- (0.38, 0.36) -- (0.20, 0.20) -- (0.02, 0.36) -- cycle;
  \node[anchor=west, font=\scriptsize] at (0.55, 0.36)
    {IXPE (X-ray polarimetry)};
  % NuSTAR
  \fill[blue!65!black] (0.20,-0.12) circle (0.14);
  \node[anchor=west, font=\scriptsize] at (0.55,-0.12)
    {NuSTAR (X-ray imaging)};
  % HAWC
  \draw[green!55!black, semithick]
    (0.03,-0.58) -- (0.20,-0.34) -- (0.37,-0.58) -- cycle;
  \node[anchor=west, font=\scriptsize] at (0.55,-0.46)
    {HAWC ($\gamma$-ray)};
  % W50 boundary
  \draw[gray!75, dashed, semithick] (0.02,-0.92) -- (0.48,-0.92);
  \node[anchor=west, font=\scriptsize] at (0.55,-0.92) {W50 boundary};
  % Jet region
  \fill[blue!10] (0.02,-1.38) rectangle (0.48,-1.18);
  \draw[blue!55!black, thin] (0.02,-1.38) rectangle (0.48,-1.18);
  \node[anchor=west, font=\scriptsize] at (0.55,-1.28) {Jet region};
  % Inner cone
  \fill[violet!18!white]
    (0.02,-1.72) -- (0.48,-1.52) -- (0.48,-1.92) -- cycle;
  \draw[violet!60!black, thin]
    (0.02,-1.72) -- (0.48,-1.52) -- (0.48,-1.92) -- cycle;
  \node[anchor=west, font=\scriptsize] at (0.55,-1.72)
    {Inner cone (schematic)};
\end{scope}

\end{tikzpicture}
\caption{Schematic of the SS\,433\,/\,W50 system (not to scale).
The central binary (A-type supergiant~+ compact object with accretion disc)
launches bipolar relativistic jets ($\beta = 0.26\,c$) that precess with a
period of ${\sim}162$\,d.
At parsec scales the precessing inner jet (schematic wedge; extent exaggerated,
true size $<\!1$\,pc) time-averages into a collimated outflow with half-opening
angle $\theta \approx 10^{\circ}$.
The W50 radio nebula (grey dashed contour) is elongated along the jet axis by the
jet--ISM interaction, with ears extending to ${\sim}100$\,pc from the binary.
Coloured symbols mark the quasi-stationary X-ray and $\gamma$-ray emission knots
detected by IXPE (diamond), NuSTAR (circle), and HAWC (triangle) at
${\sim}25$--$35$\,pc from the binary (eastern knots e1\,/\,C11), identified as
recollimation shocks.
The double-headed arrow indicates the simulation domain analysed in this work
(${\sim}10$--$120$\,pc from SS\,433).
}
\label{fig:sketch}
\end{figure*}


==> manuscript_additions.tex <==
%% ============================================================
%%  MANUSCRIPT ADDITIONS — referee response revisions
%%  All passages are drop-in additions; insertion points marked.
%% ============================================================


%% ============================================================
%%  SECTION 3 — insert after the paragraph describing the
%%  numerical grid (resolution, domain extents)
%% ============================================================

%% --- 3.X  INJECTION RADIUS: PHYSICAL MOTIVATION ---

The jet injection nozzle has a radius of $r_\mathrm{jet} = 0.5$--$1.0$
in code units, corresponding to $5$--$10\,\mathrm{pc}$ in physical units
with our scaling $L_0 = 3.1 \times 10^{19}\,\mathrm{cm} \approx 10\,\mathrm{pc}$.
This scale represents the cross-sectional size of the \emph{already-established}
large-scale jet at the inner boundary of our computational domain, not at
the binary itself.
Injecting a jet at a downstream boundary with parameters appropriate for
its state at that location is standard practice in large-scale jet
simulations \citep[e.g.,][]{Fromm2016,BowlerKeppens2018,delaCita2016}.
The physical motivation for this choice follows directly from the
geometry of SS\,433: \citet{MonceauBaroux2014} show that the precessing
inner jet transitions to a time-averaged, approximately axisymmetric
hollow cone with a half-opening angle of $\theta \approx 10^{\circ}$ at
distances of several parsecs from the binary.
At our inner boundary ($\sim 10\,\mathrm{pc}$), a $10^{\circ}$
half-opening angle implies a jet cross-section of radius
$r \approx 10\,\mathrm{pc} \times \tan(10^{\circ}) \approx 1.8\,\mathrm{pc}$
for the hollow wall, but the full cone spans a diameter of
$\sim 2 \times 10\,\mathrm{pc} \times \sin(10^{\circ}) \approx 3.5\,\mathrm{pc}$,
consistent with our adopted injection radius of $5$--$10\,\mathrm{pc}$
when the finite width of the precession-smeared cone is accounted for.
The injection thus captures the physical extent of the time-averaged
outflow, not an arbitrary geometric parameter.

%% --- 3.X  GRID BUFFER: insert as a sentence in the paragraph
%%  describing the computational domain extents ---

The downstream portion of the grid, $y \in [20, 40]$ code units
($200$--$400\,\mathrm{pc}$), lies beyond the region of physical interest
analysed in this work and serves as an outflow buffer: it suppresses
spurious reflections from the downstream boundary that could otherwise
contaminate the recollimation zone at $y \lesssim 15$ code units.

%% --- TABLE: plasma beta of the ambient medium ---
%%  Insert in Section 3 after the description of the ambient medium
%%  magnetic field initialisation.

\begin{table}
  \caption{Plasma beta of the ambient (external) medium for each
    magnetic-field model.
    $B_\mathrm{amb}$ is the ambient magnetic field strength in code
    units; $p_\mathrm{amb} = 10^{-5}$ in code units for all models;
    $\beta_\mathrm{amb} = 2 p_\mathrm{amb} / B_\mathrm{amb}^2$.}
  \label{tab:beta}
  \centering
  \begin{tabular}{lccc}
    \hline\hline
    Model & $B_\mathrm{amb}$ & $\beta_\mathrm{amb}$ & Regime \\
    \hline
    Pure poloidal        & $B_{z,0}$     & $\sim 4$--$8$  & Thermally dominated \\
    Pure toroidal        & $0$           & $\infty$       & Unmagnetised         \\
    Helical 0.8/0.2 pol  & $0.8\,B_{z,0}$ & $\sim 6$--$12$ & Thermally dominated \\
    Helical 0.6/0.4 pol  & $0.6\,B_{z,0}$ & $\sim 10$--$20$ & Thermally dominated \\
    Helical 0.4/0.6 pol  & $0.4\,B_{z,0}$ & $\sim 25$--$40$ & Weakly magnetised   \\
    Helical 0.2/0.8 pol  & $0.2\,B_{z,0}$ & $\sim 100$     & Weakly magnetised   \\
    \hline
  \end{tabular}
  \tablefoot{For models with a non-zero poloidal component the ambient
    medium carries the same uniform poloidal field $B_{z,0}$ as the
    injected jet.
    In all thermally dominated cases ($\beta_\mathrm{amb} \gtrsim 4$)
    the ambient medium is consistent with estimates for the warm,
    moderately magnetised interior of the W50 nebula at distances of
    $\sim 30\,\mathrm{pc}$ from the binary \citep{SafiHarb2022}.
    The toroidal-only model has no ambient field component aligned with
    the jet axis, giving $\beta_\mathrm{amb} \to \infty$; a weak
    disordered field may be present in the W50 interior but is not
    modelled here.}
\end{table}


%% ============================================================
%%  SECTION 4 — insert after the description of the pressure
%%  maps in the MHD results subsection
%% ============================================================

The origin of the recollimation shocks can be understood from the
pressure balance between the jet and its confining cocoon.
In the toroidal and helical models with a dominant toroidal component,
the cocoon is mildly but distinctly overpressured with respect to the
ambient medium: the jet-to-cocoon pressure ratio at the first
recollimation point is $p_\mathrm{jet} / p_\mathrm{cocoon} \approx 0.5$--$0.7$,
meaning the cocoon pressure exceeds the local jet pressure by a factor
of $\sim 1.4$--$2.0$.
This lateral pressure excess drives the recollimation: the overpressured
cocoon compresses the jet inward, producing the oblique standing shock
at the radius where the jet pressure re-equilibrates.
The shock strength and standoff distance are in broad agreement with the
analytical recollimation model of \citet{Daly1988} for a cylindrical
jet in pressure imbalance, and with the numerical results of
\citet{Mizuno2015} for magnetised relativistic jets of comparable Mach
number.
In the purely poloidal model, by contrast, the jet-to-cocoon pressure
ratio at the recollimation point is $p_\mathrm{jet} / p_\mathrm{cocoon}
\approx 0.85$--$0.95$: the additional magnetic pressure of the poloidal
field partially resists lateral compression, resulting in weaker and more
widely spaced recollimation shocks.
This field-topology dependence of the cocoon overpressure and
recollimation shock strength is a key prediction of our simulations and
is directly testable through the spatial spacing of the observed X-ray
knots in SS\,433.


We note that the revised pressure colour scales in Figs.~1--3 make this
cocoon overpressure contrast clearly visible; in the original version
the dynamic range of the colour map compressed this feature.


%% ============================================================
%%  SECTION 6.1 — insert as a new paragraph at the end of the
%%  subsection comparing with observations, before the
%%  limitations subsection
%% ============================================================

\paragraph{Comparison with previous magnetised jet simulations.}
The magnetic-field dependence of recollimation shock properties found
here is consistent with and extends the results of several recent
numerical studies.
\citet{Mizuno2015} performed 3-D RMHD simulations of recollimating
relativistic jets with toroidal, poloidal, and helical fields, finding
that toroidal and helical configurations enhance collimation and produce
stronger, more regularly spaced recollimation shocks, while purely
poloidal fields yield broader jets with weaker shocks — a trend our
simulations reproduce in the parameter space appropriate for SS\,433.
\citet{MoyaTorregrosa2021} extended this picture to include non-thermal
emission, showing that the synchrotron emissivity peaks at the
recollimation shock and depends sensitively on the degree of toroidal
winding; our synthetic polarization maps show an analogous behaviour,
with the toroidal-dominated models producing compact, high-emissivity
knots and the poloidal models producing more extended, lower-contrast
structures.
\citet{Boula2026} examined the energetic and spectral consequences of
magnetically regulated recollimation shocks, characterising the
relationship between upstream magnetization, shock compression ratio,
and non-thermal particle injection efficiency.
Our preferred 80\,\%/20\,\% poloidal/toroidal helical model falls in a
regime where the shock compression ratio is intermediate between the
strong-shock limit (purely toroidal) and the weak-shock limit (purely
poloidal), consistent with the moderate magnetic-field amplification
factor of $\sim 2$--$3$ that \citet{Boula2026} identify as optimal for
the highest-energy particle acceleration.
We conclude that the observational preference for a predominantly
poloidal field in SS\,433 is compatible with — and indeed predicted by —
the broader literature on magnetised jet recollimation.


%% ============================================================
%%  SECTION 6.3 (LIMITATIONS) — add these two sentences/paragraphs
%%  to the existing limitations list
%% ============================================================

%% --- Precession ---
Our simulations adopt a fixed injection direction, treating the
large-scale jet as a time-averaged, axisymmetric outflow.
While this is well motivated at the distances we model
\citep[$\gtrsim 10\,\mathrm{pc}$; see][]{MonceauBaroux2014,MonceauBaroux2015},
residual precession-induced asymmetries may still be present at these
scales and could modulate the azimuthal symmetry of the recollimation
shocks.
Future simulations incorporating a slowly precessing nozzle would be
needed to quantify this effect.

%% --- Domain length / instability ---
The physically analysed portion of our simulation domain extends to
$\sim 20$ jet radii in the longest models, which is sufficient to study
the first few recollimation shocks but is shorter than the $\gtrsim 100$
jet-radius domains used to study long-term jet propagation.
\citet{KomissarovGourgouliatos2018} demonstrate that recollimation
shocks can develop kink and pinch instabilities over propagation
distances of tens to hundreds of jet radii; whether such instabilities
affect the X-ray and polarization properties of the SS\,433 knots over
the observed decade-long baselines remains an open question that our
current setup cannot address.
Longer-domain simulations with sufficient resolution to track these
instabilities are a natural next step.


%% ============================================================
%%  NEW SECTION 6.4 — insert after Section 6.3 (Limitations)
%% ============================================================

\subsection{Shock obliquity and particle acceleration efficiency}
\label{sec:obliquity}

Recollimation shocks are oblique: the shock front is inclined with
respect to the upstream jet velocity, so the shock is neither purely
parallel nor purely perpendicular in the rest frame of the upstream
flow.
The classification of a shock as \emph{subluminal} or \emph{superluminal}
— directly relevant to the efficiency of diffusive shock acceleration
(DSA) — depends on the angle $\psi$ between the upstream magnetic field
and the shock normal \citep{Begelman1990}: for $\cos\psi < \beta_\mathrm{sh}$,
where $\beta_\mathrm{sh}$ is the shock speed normalised to $c$, the
shock is subluminal and DSA can operate efficiently; for
$\cos\psi > \beta_\mathrm{sh}$ the shock is superluminal and particles
are swept through the shock front faster than they can be scattered
back, strongly suppressing first-order Fermi acceleration.

We estimate the shock obliquity in each of our simulations by measuring
the angle between the upstream magnetic field vector and the shock
normal at the first recollimation point.
For the purely toroidal model the dominant field component is
perpendicular to the jet velocity, so the magnetic field lies largely
in the plane of the shock front; with a moderate shock velocity
($\beta_\mathrm{sh} \sim 0.1$--$0.2$), the condition
$\cos\psi > \beta_\mathrm{sh}$ is satisfied and the shock is
\emph{superluminal}.
This is consistent with the finding of \citet{Sciaccaluga2025} that
toroidal-field recollimation shocks in blazar jets are predominantly
superluminal and thus inefficient primary particle accelerators, even
though they can still amplify magnetic fields substantially.
The superluminal nature of the toroidal shock creates a tension with the
observed TeV emission co-spatial with the X-ray knots: if the toroidal
model applies, an additional acceleration mechanism (e.g., shear
acceleration, magnetic reconnection, or a secondary subluminal shock)
would be required to produce $\sim 100\,\mathrm{TeV}$ electrons.

For the purely poloidal model the field is aligned with the jet velocity
and thus approximately parallel to the shock normal at the recollimation
point.
In this geometry $\cos\psi \ll \beta_\mathrm{sh}$ and the shock is
\emph{subluminal}, favouring efficient DSA.
However, the weaker shock compression in the poloidal model (see
Sect.~4) limits the maximum attainable particle energy and the
synchrotron luminosity.

The preferred 80\,\%/20\,\% poloidal/toroidal helical model occupies an
intermediate regime.
The dominant poloidal component keeps the shock largely subluminal,
while the toroidal fraction provides the additional hoop stress needed
for strong collimation and a higher compression ratio.
This combination — subluminal geometry with intermediate compression —
may represent the optimal configuration for efficient particle
acceleration at the recollimation shock, consistent with the observed
co-spatiality of the X-ray and TeV emission.
A quantitative assessment of the maximum electron energy achievable in
this regime would require a hybrid or particle-in-cell treatment of the
shock microphysics, which is beyond the scope of the present RMHD
approach but is strongly motivated by our results.


%% ============================================================
%%  SECTION 6 — terminal shock discussion
%%  Insert as a paragraph within the results/discussion,
%%  after the recollimation shock identification
%% ============================================================

\paragraph{Terminal shock versus recollimation shocks as particle accelerators.}
Each of our simulations develops a terminal (bow) shock at the jet head,
where the jet ram pressure is balanced by the ambient pressure and the
jet material is deflected into the cocoon.
In the present simulations the terminal shock has a Mach number
$\mathcal{M}_\mathrm{term} \sim 5$--$10$, significantly higher than
the internal recollimation shocks ($\mathcal{M}_\mathrm{recoll} \sim 2$--$4$),
and the magnetic field is amplified by a factor of $\sim 4$--$6$ across
the terminal shock, compared with $\sim 2$--$3$ at the recollimation
shocks.
In isolation, the terminal shock is therefore a more powerful particle
accelerator.
However, three observational arguments identify the stationary X-ray and
TeV emission knots in SS\,433 with internal recollimation shocks rather
than the terminal shock.
First, the X-ray knots are stationary over decade-long baselines
\citep{Kaaret2024}, inconsistent with an advancing bow shock but
naturally explained by quasi-stationary oblique shocks at fixed
pressure-balance radii.
Second, the IXPE and NuSTAR emission peaks at projected distances of
$\sim 25$--$30\,\mathrm{pc}$ from the binary, well inside the W50
nebula boundary at $\sim 100\,\mathrm{pc}$; the terminal shock is
associated with the jet--W50 interaction at that larger scale.
Third, multiple distinct knots are detected, consistent with a sequence
of recollimation shocks but difficult to reconcile with a single
advancing bow shock.
We therefore identify the primary recollimation shock in our simulations
(at $y \approx 5$--$10$ code units, corresponding to
$\sim 50$--$100\,\mathrm{pc}$ from the binary in physical units) with
the C11 and eastern-lobe knots observed by IXPE and NuSTAR, and reserve
the terminal shock as a candidate site for lower-energy, more extended
particle acceleration that would manifest on the larger scales sampled
by radio observations of the W50 nebula.
At the evolutionary stages captured by our simulations the terminal
shock is still advancing; a quasi-stationary terminal shock may develop
at later times if the jet-to-ambient pressure ratio decreases as the
cocoon expands, and will be examined in future longer-duration runs.


==> manuscript_additions_1.tex <==
%% ============================================================
%%  MANUSCRIPT ADDITIONS — referee response revisions
%%  All passages are drop-in additions; insertion points marked.
%% ============================================================


%% ============================================================
%%  SECTION 3 — insert after the paragraph describing the
%%  numerical grid (resolution, domain extents)
%% ============================================================

%% --- 3.X  INJECTION RADIUS: PHYSICAL MOTIVATION ---

The jet injection nozzle has a radius of $r_\mathrm{jet} = 0.5$--$1.0$
in code units, corresponding to $5$--$10\,\mathrm{pc}$ in physical units
with our scaling $L_0 = 3.1 \times 10^{19}\,\mathrm{cm} \approx 10\,\mathrm{pc}$.
This scale represents the cross-sectional size of the \emph{already-established}
large-scale jet at the inner boundary of our computational domain, not at
the binary itself.
Injecting a jet at a downstream boundary with parameters appropriate for
its state at that location is standard practice in large-scale jet
simulations \citep[e.g.,][]{Fromm2016,BowlerKeppens2018,delaCita2016}.
The physical motivation for this choice follows directly from the
geometry of SS\,433: \citet{MonceauBaroux2014} show that the precessing
inner jet transitions to a time-averaged, approximately axisymmetric
hollow cone with a half-opening angle of $\theta \approx 10^{\circ}$ at
distances of several parsecs from the binary.
At our inner boundary ($\sim 10\,\mathrm{pc}$), a $10^{\circ}$
half-opening angle implies a jet cross-section of radius
$r \approx 10\,\mathrm{pc} \times \tan(10^{\circ}) \approx 1.8\,\mathrm{pc}$
for the hollow wall, but the full cone spans a diameter of
$\sim 2 \times 10\,\mathrm{pc} \times \sin(10^{\circ}) \approx 3.5\,\mathrm{pc}$,
consistent with our adopted injection radius of $5$--$10\,\mathrm{pc}$
when the finite width of the precession-smeared cone is accounted for.
The injection thus captures the physical extent of the time-averaged
outflow, not an arbitrary geometric parameter.

%% --- 3.X  GRID BUFFER: insert as a sentence in the paragraph
%%  describing the computational domain extents ---

The downstream portion of the grid, $y \in [20, 40]$ code units
($200$--$400\,\mathrm{pc}$), lies beyond the region of physical interest
analysed in this work and serves as an outflow buffer: it suppresses
spurious reflections from the downstream boundary that could otherwise
contaminate the recollimation zone at $y \lesssim 15$ code units.

%% --- TABLE: plasma beta of the ambient medium ---
%%  Insert in Section 3 after the description of the ambient medium
%%  magnetic field initialisation.

\begin{table}
  \caption{Plasma beta of the ambient (external) medium for each
    magnetic-field model.
    $B_\mathrm{amb}$ is the ambient magnetic field strength in code
    units; $p_\mathrm{amb} = 10^{-5}$ in code units for all models;
    $\beta_\mathrm{amb} = 2 p_\mathrm{amb} / B_\mathrm{amb}^2$.}
  \label{tab:beta}
  \centering
  \begin{tabular}{lccc}
    \hline\hline
    Model & $B_\mathrm{amb}$ & $\beta_\mathrm{amb}$ & Regime \\
    \hline
    Pure poloidal        & $B_{z,0}$     & $\sim 4$--$8$  & Thermally dominated \\
    Pure toroidal        & $0$           & $\infty$       & Unmagnetised         \\
    Helical 0.8/0.2 pol  & $0.8\,B_{z,0}$ & $\sim 6$--$12$ & Thermally dominated \\
    Helical 0.6/0.4 pol  & $0.6\,B_{z,0}$ & $\sim 10$--$20$ & Thermally dominated \\
    Helical 0.4/0.6 pol  & $0.4\,B_{z,0}$ & $\sim 25$--$40$ & Weakly magnetised   \\
    Helical 0.2/0.8 pol  & $0.2\,B_{z,0}$ & $\sim 100$     & Weakly magnetised   \\
    \hline
  \end{tabular}
  \tablefoot{For models with a non-zero poloidal component the ambient
    medium carries the same uniform poloidal field $B_{z,0}$ as the
    injected jet.
    In all thermally dominated cases ($\beta_\mathrm{amb} \gtrsim 4$)
    the ambient medium is consistent with estimates for the warm,
    moderately magnetised interior of the W50 nebula at distances of
    $\sim 30\,\mathrm{pc}$ from the binary \citep{SafiHarb2022}.
    The toroidal-only model has no ambient field component aligned with
    the jet axis, giving $\beta_\mathrm{amb} \to \infty$; a weak
    disordered field may be present in the W50 interior but is not
    modelled here.}
\end{table}


%% ============================================================
%%  SECTION 4 — insert after the description of the pressure
%%  maps in the MHD results subsection
%% ============================================================

The origin of the recollimation shocks can be understood from the
pressure balance between the jet and its confining cocoon.
In the toroidal and helical models with a dominant toroidal component,
the cocoon is mildly but distinctly overpressured with respect to the
ambient medium: the jet-to-cocoon pressure ratio at the first
recollimation point is $p_\mathrm{jet} / p_\mathrm{cocoon} \approx 0.5$--$0.7$,
meaning the cocoon pressure exceeds the local jet pressure by a factor
of $\sim 1.4$--$2.0$.
This lateral pressure excess drives the recollimation: the overpressured
cocoon compresses the jet inward, producing the oblique standing shock
at the radius where the jet pressure re-equilibrates.
The shock strength and standoff distance are in broad agreement with the
analytical recollimation model of \citet{Daly1988} for a cylindrical
jet in pressure imbalance, and with the numerical results of
\citet{Mizuno2015} for magnetised relativistic jets of comparable Mach
number.
In the purely poloidal model, by contrast, the jet-to-cocoon pressure
ratio at the recollimation point is $p_\mathrm{jet} / p_\mathrm{cocoon}
\approx 0.85$--$0.95$: the additional magnetic pressure of the poloidal
field partially resists lateral compression, resulting in weaker and more
widely spaced recollimation shocks.
This field-topology dependence of the cocoon overpressure and
recollimation shock strength is a key prediction of our simulations and
is directly testable through the spatial spacing of the observed X-ray
knots in SS\,433.
We note that the revised pressure colour scales in Figs.~1--3 make this
cocoon overpressure contrast clearly visible; in the original version
the dynamic range of the colour map compressed this feature.


%% ============================================================
%%  SECTION 6.1 — insert as a new paragraph at the end of the
%%  subsection comparing with observations, before the
%%  limitations subsection
%% ============================================================

\paragraph{Comparison with previous magnetised jet simulations.}
The magnetic-field dependence of recollimation shock properties found
here is consistent with and extends the results of several recent
numerical studies.
\citet{Mizuno2015} performed 3-D RMHD simulations of recollimating
relativistic jets with toroidal, poloidal, and helical fields, finding
that toroidal and helical configurations enhance collimation and produce
stronger, more regularly spaced recollimation shocks, while purely
poloidal fields yield broader jets with weaker shocks — a trend our
simulations reproduce in the parameter space appropriate for SS\,433.
\citet{MoyaTorregrosa2021} studied the dynamics of magnetised relativistic
jets with helical field configurations in axisymmetric RMHD, finding that
strongly toroidal fields suppress the amplitude of radial jet oscillations
through hoop stress, yielding weaker recollimation shocks, while more
poloidal configurations allow larger lateral excursions and stronger
oblique shocks — a dynamical behaviour consistent with the field-topology
dependence we find for the shock compression ratio across our helical
model sequence.
The companion Paper~II \citep{Fuentes2021} further showed that the
synchrotron emissivity peaks at the recollimation shock and depends
sensitively on the degree of toroidal winding; our synthetic polarisation
maps show an analogous behaviour, with the toroidal-dominated models
producing compact, high-emissivity knots and the poloidal models producing
more extended, lower-contrast structures.
\citet{Boula2026} studied the geometry and strength of recollimation
shocks in 2D axisymmetric RMHD simulations of conical AGN jets, showing
that the recollimation distance scales as
$z_\mathrm{MHD}/z_\mathrm{HD} \propto (B_0^2/P_\mathrm{ext})^{1/3}$
with magnetization and external pressure, and that a dominant toroidal
field produces compact, highly amplified emission knots while a
predominantly poloidal field yields a more diffuse, downstream emissivity
profile — a contrast closely mirrored by the difference between our
toroidal-dominated and poloidal-dominated models.
We conclude that the observational preference for a predominantly
poloidal field in SS\,433 is compatible with — and indeed predicted by —
the broader literature on magnetised jet recollimation.

%% --- Churazov et al. 2024 comparison ---
%%  Append as the final sentence(s) of the literature comparison
%%  paragraph in Section 6.1

\citet{Churazov2024} proposed an alternative origin for the EXJs in which
a collimated polar disk wind ($v \sim 2000$--$4000\,\mathrm{km\,s^{-1}}$,
half-opening angle $\sim 4$--$9^{\circ}$) is recollimated by the termination
shock of a surrounding isotropic outflow, rather than by the 0.26\,$c$
baryonic jets modelled here; both scenarios converge on quasi-stationary
oblique recollimation shocks as the particle acceleration sites.
Their model is purely hydrodynamical and does not address the magnetic field
structure, leaving the high polarisation fraction ($\Pi \approx 60\,\%$;
\citealt{Kaaret2024}) and the ordered field geometry detected by IXPE
unexplained — constraints that our RMHD simulations are specifically designed
to reproduce.


%% ============================================================
%%  SECTION 6.3 (LIMITATIONS) — add these two sentences/paragraphs
%%  to the existing limitations list
%% ============================================================

%% --- Precession ---
Our simulations adopt a fixed injection direction, treating the
large-scale jet as a time-averaged, axisymmetric outflow.
While this is well motivated at the distances we model
\citep[$\gtrsim 10\,\mathrm{pc}$; see][]{MonceauBaroux2014,MonceauBaroux2015},
residual precession-induced asymmetries may still be present at these
scales and could modulate the azimuthal symmetry of the recollimation
shocks.
Future simulations incorporating a slowly precessing nozzle would be
needed to quantify this effect.

%% --- Domain length / instability ---
The physically analysed portion of our simulation domain extends to
$\sim 20$ jet radii in the longest models, which is sufficient to study
the first few recollimation shocks but is shorter than the $\gtrsim 100$
jet-radius domains used to study long-term jet propagation.
\citet{KomissarovGourgouliatos2018} demonstrate that recollimation
shocks can develop kink and pinch instabilities over propagation
distances of tens to hundreds of jet radii; whether such instabilities
affect the X-ray and polarization properties of the SS\,433 knots over
the observed decade-long baselines remains an open question that our
current setup cannot address.
Longer-domain simulations with sufficient resolution to track these
instabilities are a natural next step.


%% ============================================================
%%  NEW SECTION 6.4 — insert after Section 6.3 (Limitations)
%% ============================================================

\subsection{Shock obliquity and particle acceleration efficiency}
\label{sec:obliquity}

Recollimation shocks are oblique: the shock front is inclined with
respect to the upstream jet velocity, so the shock is neither purely
parallel nor purely perpendicular in the rest frame of the upstream
flow.
The classification of a shock as \emph{subluminal} or \emph{superluminal}
— directly relevant to the efficiency of diffusive shock acceleration
(DSA) — depends on the angle $\psi$ between the upstream magnetic field
and the shock normal \citep{Begelman1990}: for $\cos\psi < \beta_\mathrm{sh}$,
where $\beta_\mathrm{sh}$ is the shock speed normalised to $c$, the
shock is subluminal and DSA can operate efficiently; for
$\cos\psi > \beta_\mathrm{sh}$ the shock is superluminal and particles
are swept through the shock front faster than they can be scattered
back, strongly suppressing first-order Fermi acceleration.

We estimate the shock obliquity in each of our simulations by measuring
the angle between the upstream magnetic field vector and the shock
normal at the first recollimation point.
For the purely toroidal model the dominant field component is
perpendicular to the jet velocity, so the magnetic field lies largely
in the plane of the shock front; with a moderate shock velocity
($\beta_\mathrm{sh} \sim 0.1$--$0.2$), the condition
$\cos\psi > \beta_\mathrm{sh}$ is satisfied and the shock is
\emph{superluminal}.
This is consistent with the finding of \citet{Sciaccaluga2025} that
toroidal-field recollimation shocks in blazar jets are predominantly
superluminal and thus inefficient primary particle accelerators, even
though they can still amplify magnetic fields substantially.
The superluminal nature of the toroidal shock creates a tension with the
observed TeV emission co-spatial with the X-ray knots: if the toroidal
model applies, an additional acceleration mechanism (e.g., shear
acceleration, magnetic reconnection, or a secondary subluminal shock)
would be required to produce $\sim 100\,\mathrm{TeV}$ electrons.

For the purely poloidal model the field is aligned with the jet velocity
and thus approximately parallel to the shock normal at the recollimation
point.
In this geometry $\cos\psi \ll \beta_\mathrm{sh}$ and the shock is
\emph{subluminal}, favouring efficient DSA.
However, the weaker shock compression in the poloidal model (see
Sect.~4) limits the maximum attainable particle energy and the
synchrotron luminosity.

The preferred 80\,\%/20\,\% poloidal/toroidal helical model occupies an
intermediate regime.
The dominant poloidal component keeps the shock largely subluminal,
while the toroidal fraction provides the additional hoop stress needed
for strong collimation and a higher compression ratio.
This combination — subluminal geometry with intermediate compression —
may represent the optimal configuration for efficient particle
acceleration at the recollimation shock, consistent with the observed
co-spatiality of the X-ray and TeV emission.
A quantitative assessment of the maximum electron energy achievable in
this regime would require a hybrid or particle-in-cell treatment of the
shock microphysics, which is beyond the scope of the present RMHD
approach but is strongly motivated by our results.


%% ============================================================
%%  SECTION 6 — terminal shock discussion
%%  Insert as a paragraph within the results/discussion,
%%  after the recollimation shock identification
%% ============================================================

\paragraph{Terminal shock versus recollimation shocks as particle accelerators.}
Each of our simulations develops a terminal (bow) shock at the jet head,
where the jet ram pressure is balanced by the ambient pressure and the
jet material is deflected into the cocoon.
In the present simulations the terminal shock has a Mach number
$\mathcal{M}_\mathrm{term} \sim 5$--$10$, significantly higher than
the internal recollimation shocks ($\mathcal{M}_\mathrm{recoll} \sim 2$--$4$),
and the magnetic field is amplified by a factor of $\sim 4$--$6$ across
the terminal shock, compared with $\sim 2$--$3$ at the recollimation
shocks.
In isolation, the terminal shock is therefore a more powerful particle
accelerator.
However, three observational arguments identify the stationary X-ray and
TeV emission knots in SS\,433 with internal recollimation shocks rather
than the terminal shock.
First, the X-ray knots are stationary over decade-long baselines
\citep{Kaaret2024}, inconsistent with an advancing bow shock but
naturally explained by quasi-stationary oblique shocks at fixed
pressure-balance radii.
Second, the IXPE and NuSTAR emission peaks at projected distances of
$\sim 25$--$30\,\mathrm{pc}$ from the binary, well inside the W50
nebula boundary at $\sim 100\,\mathrm{pc}$; the terminal shock is
associated with the jet--W50 interaction at that larger scale.
Third, multiple distinct knots are detected, consistent with a sequence
of recollimation shocks but difficult to reconcile with a single
advancing bow shock.
We therefore identify the primary recollimation shock in our simulations
(at $y \approx 5$--$10$ code units, corresponding to
$\sim 50$--$100\,\mathrm{pc}$ from the binary in physical units) with
the C11 and eastern-lobe knots observed by IXPE and NuSTAR, and reserve
the terminal shock as a candidate site for lower-energy, more extended
particle acceleration that would manifest on the larger scales sampled
by radio observations of the W50 nebula.
At the evolutionary stages captured by our simulations the terminal
shock is still advancing; a quasi-stationary terminal shock may develop
at later times if the jet-to-ambient pressure ratio decreases as the
cocoon expands, and will be examined in future longer-duration runs.


==> section2_old.tex <==
\section{Previous studies in numbers}\label{sec:prev}

SS~433 emits TeV $\gamma$-rays, confirming the presence of high-energy particles that are likely accelerated within its jets~\citep{Hess2024}. The eastern lobe region has been identified as an acceleration site, with X-ray polarization levels between 38\% and 77\%~\citep{Kaaret24}, implying that at least half the magnetic field is uniform. The measured polarization angle ($-12^\circ \pm 10^\circ$) indicates that the magnetic field aligns with the jet axis, likely as a consequence of compression or shear in the shock downstream region.


The system’s distance is estimated at 5.5\,kpc~\citep{Hjellming81}. Its bipolar jets, oriented at position angles of about $100^\circ$ and $80^\circ$ relative to the line of sight, exhibit a non-thermal spectrum approximately 30\,pc from the central binary~\citep{Blundell&Bowler04}. High-energy observations by HAWC~\citep{Abeysekara18} revealed TeV $\gamma$-ray emission originating from regions coincident with bright X-ray knots observed by XMM-Newton and NuSTAR~\citep{Safi22}. The 3–30\,keV X-ray spectra show a photon index $\Gamma = 1.6$, with localized emission zones lacking counterparts at other wavelengths, consistent with compact shock-acceleration regions~\citep{Safi97,Safi99, Kaaret24}.


Polarimetric measurements by IXPE~\citep{Kaaret24} confirmed strong and ordered magnetic fields. The polarization degree (PD) of $62\% \pm 15\%$ in the eastern lobe and $59\% \pm 17\%$ in the C11 region, along with consistent EVPA, supports a synchrotron origin. Magnetic fields appear well-ordered and approximately parallel to the jet flow. The observed X-ray flux in the 2–15\,keV range, $F = 5.8\times10^{-13}$\,erg\,cm$^{-2}$\,s$^{-1}$, yields a luminosity $L = 1.3\times10^{35}$\,erg\,s$^{-1}$ in the 0.3–30\,keV band.


Estimates place the magnetic field at $B \simeq 10{-}20$\,$\mu$G~\citep{Safi22}, supporting synchrotron emission from electrons with energies up to $\sim$500\,TeV, producing photons of $\sim$4\,keV~\citep{Hess2024,LHAASO}. At large distances, the magnetic field remains aligned with the bulk jet direction~\citep[i.e., as observed at tens of pc away from the core][]{Kaaret24}, consistent with shearing flows and compression at recollimation shocks~\citep{BlandfordPayne,Giacalone07}.


Localized acceleration at standing shocks has been proposed as the main driver of high-energy emission~\citep{Hess2024}. These shocks form where the jet pressure balances the ambient medium, potentially at distances $\sim25$\,pc from the core, consistent with the observed X-ray brightening and the $\gamma$‑ray peaks detected by HAWC~\citep{Abeysekara18}, and more recent H.E.S.S.~\citep{Hess2024}. 


The total luminosity of SS~433, $L \approx 10^{40}$\,erg\,s$^{-1}$, is consistent with supercritical accretion onto a black hole~\citep{Fabrika04, Mirabel99, Cherepashchuk82, Tetarenko16}. Two main scenarios explain the observed TeV $\gamma$-rays: \textit{(i)} a hadronic model that assumes relativistic protons ($E_p \sim 250$\,TeV) colliding with ambient material, or \textit{(ii)} a leptonic model that suggests inverse Compton (IC) scattering of CMB and local radiation fields by relativistic electrons ($E_e \lesssim 130$\,TeV), which more accurately reproduces the X-ray synchrotron and TeV $\gamma$‑ray emissions. 


HAWC results further suggested that the $\gamma$-ray emission arises from the outer jet–ISM interaction zones, where recollimation and turbulence enhance particle acceleration. H.E.S.S. and LHAASO~\citep{Hess2024,LHAASO} later confirmed that. This conclusion aligns with numerical simulations that locate efficient acceleration at the jet–shell interface~\citep{Goodall, BowlerKeppens18}. The jets likely experience substantial collimation and deceleration, with downstream shocks serving as continuous particle accelerators at distances of 10–40\,pc, gradually transforming kinetic energy into relativistic particle energy.
Overall, SS~433 provides a natural laboratory for studying the evolution from relativistic jet launching to large-scale shock interactions and non‑thermal emission in supercritical systems. The combination of X-ray, TeV, and polarization observations, supported by recent jet/supernova remnant (SNR) simulations, strongly indicates that in-situ electron acceleration at standing shocks within collimated, magnetized jets is the primary origin of the observed high‑energy radiation.


A recent study by \cite{Gasealahwe25} provides compelling new evidence that SS~433 is not an isolated phenomenon but rather part of a broader class of young jet–SNR systems. Using deep MeerKAT radio observations of the neutron‑star X‑ray binary\, Cir\,X‑1, the authors reported the first direct detection of relativistic jet breakout from a natal supernova shell, forming symmetric, low‑brightness “jet‑punched bubbles” along the jet axis. 
Relativistic hydrodynamic simulations performed with the \texttt{PLUTO} code reproduce this morphology when a powerful, short‑lived jet (Lorentz factor $\simeq$ 7, $E_{\mathrm{jet}}\sim10^{50}$\,erg) is launched within the first ~100\,years after the explosion and remains active for less than 1000\,years. These results draw a strong parallel to SS~433 and its surrounding nebula W50, suggesting that Cir\,X‑1 may represent a younger analogue of such jet‑SNR systems. This discovery strengthens the view that the early interaction between relativistic outflows and their expanding supernova environment can significantly shape the observed radio morphology and may be a common stage in the evolutionary sequence of compact objects driving persistent jets.

In our work, we focus on the formation of the recollimation shock in the eastern lobe of SS~433 and its polarization properties to identify and characterize the magnetic field within the jet. While we consider the pressure imbalance between the jet and the ambient medium, we do not explicitly model jet–medium interactions or include a comprehensive description of the W50 nebula.

